Explicit Mutual Information Maximization for Self-Supervised Learning

Recently, self-supervised learning (SSL) has been extensively studied. Theoretically, mutual information maximization (MIM) is an optimal criterion for SSL, with a strong theoretical foundation in information theory. However, it is difficult to directly apply MIM in SSL since the data distribution is not analytically available in applications. In practice, many existing methods can be viewed as approximate implementations of the MIM criterion. This work shows that, based on the invariance property of MI, explicit MI maximization can be applied to SSL under a generic distribution assumption, i.e., a relaxed condition of the data distribution. We further illustrate this by analyzing the generalized Gaussian distribution. Based on this result, we derive a loss function based on the MIM criterion using only second-order statistics. We implement the new loss for SSL and demonstrate its effectiveness via extensive experiments.

==> contents/Append.tex <==
 % \section*{Appendices} \label{sec:append}


\section{Ablation Study}  \label{app:Ablation}
\paragraph{Batch size.}
%%%% 如果加了momentum的结果，是不是最好再加上BYOL或是其他基于非对称结构进行训练的结果？
To evaluate the robustness of our method against batch size, we train the model on CIFAR -100 and ImageNet-100 with different batch sizes, following the same training setting as described in Section \ref{sec:linear}. The learning rate is adjusted following a linear scaling rule \cite{goyalAccurateLargeMinibatch2018}. 
We consider two variants of our method, one is standard and the
other uses a momentum encoder \cite{grillBootstrapYourOwn2020,chenExploringSimpleSiamese2020}.
As shown in Table \ref{tab:abl_bs}, both our method and Barlow Twins reach a saturation point as batch size increases, which is consistent with the results in \cite{zbontarBarlowTwinsSelfSupervised2021,zhangZEROCLINSTANCEFEATURE2022}. Our method has better robustness across varying batch sizes, with a maximum accuracy variation of 1.6\% on CIFAR-100 and 2.0\% on ImageNet-100, respectively, while Barlow Twins shows 5.6\% and 2.9\% accuracy variation on the two datasets. For our method, using a momentum encoder helps to enhance performance across different batch sizes.

  %\vspace{- \baselineskip}
\begin{table}[h]
    %\vspace{- 2 mm}
% \vspace{- \baselineskip}
  % \vspace{\baselineskip} % 在标题前添加近似单行间距
  \caption{\textbf{Robustness to batch size.} 
  We use the same setup as in Table \ref{tab:CIFAR_linear} but vary the batch size. "Ours-M" denotes our method with a momentum encoder. %We follow the linear scaling rule \cite{goyalAccurateLargeMinibatch2018} to adjust the learning rate and report the top Acc@1 result. "Ours" refers to our standard Siamese network setup, while "Ours-M" denotes our training structure utilizing a momentum encoder.
  }
    \vspace{\baselineskip} % 在标题前添加近似单行间距
  \label{tab:abl_bs}
  \centering
  \begin{tabular}{ccccccc}
    \toprule
    Batch size & \multicolumn{3}{c}{CIFAR-100} & \multicolumn{3}{c}{ImageNet-100} \\
    \cmidrule(r){2-4} \cmidrule(r){5-7}
     & Ours & Ours-M& Barlow Twins& Ours & Ours-M& Barlow Twins\\
    \midrule
    1024 & 68.9 & 70.4 & 65.9 & 79.8 & 81.4 & 77.5 \\
    512 & 70.0 & 70.5 & 68.7 & 79.5 & 81.1& 79.6 \\
    256 & 70.5 & 70.4 & 70.9 & 81.1 & 81.7 & 80.4 \\
    128 & 70.2 & 70.2 & 71.5 & 80.7 & 81.8 & 80.2 \\
    64 & 70.1 & 71.1 & 70.2 & 79.1 & 81.2 & 78.4 \\
    \bottomrule
  \end{tabular}
\end{table}
  % \vspace{- \baselineskip}
% \begin{table}[h]
%   \caption{\textbf{Robustness to Batch Size.} We adopt the same experimental settings as in Table \ref{tab:CIFAR_linear} but with different batch sizes.   We report the top Acc@1 result.  "Ours" denotes our Siamese network configuration, while "Ours-M" indicates our asymmetric training structure utilizing a momentum encoder.}
%   \label{tab:abl_bs}
%   \centering
%   \begin{tabular}{ccccccc}
%     \toprule
%     Batch Size & \multicolumn{3}{c}{CIFAR-100} & \multicolumn{3}{c}{ImageNet-100} \\
%     \cmidrule(r){2-4} \cmidrule(r){5-7}https://latex.sjtu.edu.cn/project/664716968562f2a4068bec21
%      & Ours & Ours-M& Barlow & Ours & Ours-M& Barlow \\
%     \midrule
%     1024 & 68.9 & 70.37 & 65.87 & 79.76 & 81.42 & 77.52 \\
%     512 & 70.01 & 70.48 & 68.73 & 79.48 & 81.0& 79.6 \\
%     256 & 70.49 & 70.41 & 70.9 & 81.1 & 81.7 & 80.38 \\
%     128 & 70.17 & 70.21 & 71.5 & 80.72 & 81.84 & 80.24 \\
%     64 & 70.08 & 71.13 & 70.23 & 79.1 & 81.2 & 78.44 \\
%     \bottomrule
%   \end{tabular}
% \end{table}
\paragraph{Loss function.}
We investigate the effectiveness of each term of the loss function (\ref{SSL_MMI_formulation3}). Specifically, we remove one of $\log{\operatorname{det}{C_{ZZ}}}$ term (w/o $\log{\operatorname{det}{C_{ZZ}}}$) and the $\log{\operatorname{det}{C_{Z'Z'}}}$ term (w/o $\log{\operatorname{det}{C_{Z'Z'}}}$) or both terms (w/o  both) from the loss function. Additionally, we replace the $\log{\operatorname{det}({C_{ZZ}-C_{Z'Z'}})}$ term with $\|Z-Z'\|^2$ since both terms aim to align the representations $Z$ and $Z'$. Furthermore, we simplify (\ref{rescaling}) from $ \tilde{M}=\frac{M-\mu_{\lambda} I}{\alpha}+I$ to $ \tilde{M}=\frac{M}{\alpha}+I$ (w/o $\mu_{\lambda}$).
Results in Table \ref{tab:abla_variants} show that removing either $\log{\operatorname{det}{C_{ZZ}}}$ or $\log{\operatorname{det}{C_{Z'Z'}}}$ leads to performance decrease, yet the training still succeed. However, removing both leads to training failure. 
\begin{table}
% \begin{wraptable}{l}{0.55\textwidth}
  % \vspace{\baselineskip} % 在标题前添加近似单行间距
  \caption{\textbf{Ablation on loss function. } The experiment follows the same setup as in Table \ref{tab:CIFAR_linear}, with Top-1 accuracy is reported. 
  }
  \vspace{\baselineskip} % 在标题前添加近似单行间距
  \label{tab:abla_variants}
  \centering
  \begin{tabular}{lcccc}
    \toprule
    Method & CIFAR-100  & ImageNet-100 \\
    \midrule
    Original & 70.5 &  81.1 \\
     w/o  $\log{\operatorname{det}{C_{ZZ}}} $ &  66.6 &  76.5 \\
     w/o  $\log{\operatorname{det}{C_{Z'Z'}}}$ & 67.7 &  78.8 \\
    w/o both & 3.55 &  4.01 \\
    Using $\|Z-Z'\|^2$ & 69.8 &  79.6 \\
         w/o  $\mu_{\lambda}$  in (\ref{rescaling})&  70.6 &  80.3 \\ %这个要删掉吗？ 感觉没什么规律 
    %z1z2\_ratio=0.1 & 70.76 & crash & 82.28 & crash \\
    \bottomrule
  \end{tabular}
  % \vspace{-4mm}
\end{table}
% \end{wraptable}
The reason behind this is straightforward. By minimizing the term $\log{\operatorname{det}({C_{ZZ}-C_{Z'Z'}})}$, we aim to align the representations $Z$ and $Z'$. The terms $\log{\operatorname{det}{C_{ZZ}}}$ and $\log{\operatorname{det}{C_{Z'Z'}}}$ play a crucial role in ensuring that these representations are informative enough to prevent representation collapse. 
When one of these terms is removed, the remaining term is expected to partially fulfill this, but becomes less effective.

It can be seen from Table \ref{tab:abla_variants} that replacing the $\log{\operatorname{det}({C_{ZZ}-C_{Z'Z'}})}$ term with $\|Z-Z'\|^2$ decreases the performance.
%From Table \ref{tab:abla_variants}, the term $\|Z-Z'\|^2$  is less effective than the original $\log{\operatorname{det}({C_{ZZ}-C_{Z'Z'}})}$ term.  
Although both $\log{\operatorname{det}({C_{ZZ}-C_{Z'Z'}})}$ and  $\|Z-Z'\|^2$ encourage consistency between $Z$ and $Z'$, their mathematical properties differ significantly. The term $\log{\operatorname{det}({C_{ZZ}-C_{Z'Z'}})}$  encourages a holistic consistency in the structural properties of the feature spaces. Meanwhile, our derived loss function obviates the need to tune the balance ratio between the terms. Moreover, the results show that removing $\mu_{\lambda}$ term in the Taylor approximation, i.e. adding a fixed $I_d$ to the three terms in the loss function does not affect the performance on CIFAR-100 but decreases the performance on ImageNet-100. 
%It can potentially allow for some individual feature discrepancies as long as the overall structural and geometric properties are preserved, while $\|Z-Z'\|^2$ enforces a strict constraint to similarity on a per-feature basis, penalizing any deviation between corresponding features.  This can have the risk of overfitting to noise or irrelevant details. What's more,  our derived loss function obviates the need to tune the ratio between $\|Z-Z'\|^2$ and the other two terms. Removing $\mu$ term, i.e. adding a fixed $I_d$ to the three terms in the loss function does not affect the performance on CIFAR-100 but decreases the performance on ImageNet-100.  %%% remove \mu的实验要删掉吗?
% \begin{table}

\paragraph{Projector hidden dimension and projector output dimension.}
We evaluate the effect of the projector's hidden dimension and projector output dimension in Table \ref{tab:abl_pj_hidden}. For both our method and Barlow Twins, there's a tendency that the increase of projector hidden dimension generally improves the performance on both the CIFAR-100 and ImageNet-100 datasets. 
Compared with CIFAR-100, both our method and Barlow Twins need a larger 
hidden dimension to achieve high performance on the more complex ImageNet-100 dataset. Using a momentum encoder, our method can achieve better performance
and becomes more robust to projector hidden dimension.
Moreover, similar to the results on the hidden dimension, 
both our method and Barlow Twins exhibit a trend that 
increasing the projector output dimension generally improves performance. 
The performance of Barlow Twins is particularly sensitive to projector output dimension, whereas our method performs well even with a very small projector output dimension of 256.  %our method can achieve better performance and becomes more robust to projector hidden dimension.

%\vspace{- \baselineskip}
  % \vspace{- \baselineskip}
\begin{table}[h]
  % \vspace{\baselineskip} % 在标题前添加近似单行间距
  \caption{\textbf{Impact of projector hidden/output dimension on accuracy.}}
    \vspace{\baselineskip} % 在标题前添加近似单行间距
  \label{tab:abl_pj_hidden}
  \centering
  \begin{tabular}{ccccccc}
    \toprule
  & \multicolumn{3}{c}{{CIFAR100}} & \multicolumn{3}{c}{{ImageNet100}} \\
  \cmidrule(r){1-4} \cmidrule(r){5-7}
        {Proj. hidden dim} & {Ours} & {Ours-M} & {Barlow Twins} & {Ours} & {Ours-M} & {Barlow Twins} \\
    \midrule
    % 2048 & 70.54 & 70.41 & 70.9 & 81.1 & 81.7 & 80.38 \\
    % 1024 & 70.84 & 70.43 & 70.17 & 80.24 & 81.46 & 79.28 \\
    % 512 & 69.14 & 70.13 & 69.58 & 79.48 & 81.36 & 78.3 \\
    % 256 & 67.85 & 70.01 & 67.96 & 78.7 & 80.6 & 76.88 \\
    2048 & 70.5 & 70.4 & 70.9 & 81.1 & 81.7 & 80.4 \\
1024 & 70.8 & 70.4 & 70.2 & 80.2 & 81.5 & 79.3 \\
512  & 69.1 & 70.1 & 69.6 & 79.5 & 81.4 & 78.3 \\
256  & 67.9 & 70.0 & 68.0 & 78.7 & 80.6 & 76.9 \\
    % \toprule
     \cmidrule(r){1-4} \cmidrule(r){5-7}
    {Proj. output dim} & {Ours} & {Ours-M} & {Barlow Twins} & {Ours} & {Ours-M} & {Barlow Twins}    \\
    \midrule
    2048 & 70.5 & 70.4 & 70.9 & 81.1 & 81.7 & 80.4 \\
1024 & 70.3 & 70.4 & 69.7 & 80.6 & 81.1 & 79.6 \\
512  & 70.6 & 70.5 & 66.5 & 80.4 & 81.7 & 77.4 \\
256  & 70.5 & 71.1 & 62.1 & 80.3 & 81.2 & 73.6 \\
\bottomrule
  \end{tabular}
\end{table}
%A larger hidden dimension allows the network to capture more complex features and relationships within the backbone outputs, potentially leading to better performance. However, beyond a certain threshold, the gains in accuracy begin to plateau, indicating that the representational capacity of the projector has exceeded the informational content of the backbone output. The fact that CIFAR-100 reaches this plateau earlier than ImageNet-100 validates the viewpoint. 
% \begin{table}[h]
%   \caption{\textbf{Impact of projector hidden dimension on accuracy.}}
%   \label{tab:abl_pj_hidden}
%   \centering
%   \begin{tabular}{ccccccc}
%     \toprule
%     {Proj. Hidden Dim} & \multicolumn{3}{c}{{CIFAR100}} & \multicolumn{3}{c}{{ImageNet100}} \\
%     \cmidrule(r){2-4} \cmidrule(r){5-7}
%      & {Ours} & {Ours-M} & {Barlow Twins} & {Ours} & {Ours-M} & {Barlow Twins} \\
%     \midrule
%     % 2048 & 70.54 & 70.41 & 70.9 & 81.1 & 81.7 & 80.38 \\
%     % 1024 & 70.84 & 70.43 & 70.17 & 80.24 & 81.46 & 79.28 \\
%     % 512 & 69.14 & 70.13 & 69.58 & 79.48 & 81.36 & 78.3 \\
%     % 256 & 67.85 & 70.01 & 67.96 & 78.7 & 80.6 & 76.88 \\
%     2048 & 70.5 & 70.4 & 70.9 & 81.1 & 81.7 & 80.4 \\
% 1024 & 70.8 & 70.4 & 70.2 & 80.2 & 81.5 & 79.3 \\
% 512  & 69.1 & 70.1 & 69.6 & 79.5 & 81.4 & 78.3 \\
% 256  & 67.9 & 70.0 & 68.0 & 78.7 & 80.6 & 76.9 \\
%     \bottomrule
%   \end{tabular}
% \end{table}


%\paragraph{Projector output dimension}
%We investigate the sensitivity of the projector's output dimension in Table \ref{tab:abl_pj_out}. The projector output dimension decides the final feature space in which the SSL loss is calculated, directly impacting the quality and characteristics of the learned representations. Similar to the analysis of the hidden dimension, both our method and Barlow Twins exhibit a trend where increasing the projector output dimension generally enhances performance. The performance of Barlow Twins is particularly sensitive to projector output dimension, whereas our method maintains effectiveness even with a smaller projector output dimension. 
% \begin{table}[h]
%   \caption{\textbf{Impact of projector output dimension on accuracy}}. 
%   \label{tab:abl_pj_out}
%   \centering
%   \begin{tabular}{ccccccc}
%     \toprule
%     {Proj. output dim} & \multicolumn{3}{c}{{CIFAR-100}} & \multicolumn{3}{c}{{ImageNet-100}} \\
%     \cmidrule(r){2-4} \cmidrule(r){5-7}
%      & {Ours} & {Ours-M} & {Barlow Twins} & {Ours} & {Ours-M} & {Barlow Twins} \\
%     \midrule
%     2048 & 70.5 & 70.4 & 70.9 & 81.1 & 81.7 & 80.4 \\
% 1024 & 70.3 & 70.4 & 69.7 & 80.6 & 81.1 & 79.6 \\
% 512  & 70.6 & 70.5 & 66.5 & 80.4 & 81.7 & 77.4 \\
% 256  & 70.5 & 71.1 & 62.1 & 80.3 & 81.2 & 73.6 \\
%     % 2048 & 70.54 & 70.41 & 70.9 & 81.1 & 81.7 & 80.38 \\
%     % 1024 & 70.29 & 70.35 & 69.74 & 80.62 & 81.06 & 79.6 \\
%     % 512 & 70.57 & 70.46 & 66.52 & 80.4 & 81.74 & 77.42 \\
%     % 256 & 70.47 & 71.06 & 62.08 & 80.3 & 81.16 & 73.6 \\
%     % 64 & - & - & 52.61 & 78.92 & - & - \\
%     \bottomrule
%   \end{tabular}
% \end{table}


% \paragraph{Ablation on predictor hidden dimension}

% \begin{table}
%   \caption{Ablation on Predictor Hidden Dimension. We use ResNet18 as backbone. The experiment}
%   \label{tab:abl_pred_hidden}
%   \centering
%   \begin{tabular}{lcc}
%     \toprule
%     Pred. Hidden Dim & CIFAR-100 & ImageNet-100\\
%     \midrule
%     1024 & 70.41 & 81.7 \\
%     512 & 69.17 & 81.28 \\
%     256 & 69.84 & 81.26 \\
%     \bottomrule
%   \end{tabular}
% \end{table}

\section{Proof of Theorem 1} \label{app:A}

We first recall the result on the invariance property of mutual information. Specifically, if $Y = F(Z)$ and $Y' = G(Z')$ are homeomorphisms, then $I(Z;Z') = I(Y;Y')$ \cite{kraskov2004estimating}. Denote $\tilde Y = {[{Y^T},{Y'^T}]^T}$, if $Y = F(Z)$ and $Y' = G(Z')$ are Gaussian distributed, i.e. $Y \sim \mathcal{N}(Y;{\mu _Y},{C_{YY}})$ and $Y' \sim \mathcal{N}(Y';{\mu _{Y'}},{C_{Y'Y'}})$, we have $\tilde Y \sim \mathcal{N}(\tilde Y;{\mu _{\tilde Y}},{C_{\tilde Y\tilde Y}})$ with 
\[{C_{\tilde Y\tilde Y}} = \left[ {\begin{array}{*{20}{c}}
{{C_{YY}}}&{{C_{YY'}}}\\
{{C_{Y'Y}}}&{{C_{Y'Y'}}}
\end{array}} \right].\]
Then, the mutual information $I(Y;Y') = H(Y) + H(Y') - H(Y,Y')$ is given by
\[I(Y;Y') = \frac{1}{2}\log \frac{{\det ({C_{YY}})\det ({C_{Y'Y'}})}}{{\det ({C_{\tilde Y\tilde Y}})}},\]
where $H(Y)$ and $H(Y')$ are the marginal entropy of $Y$ and $Y'$, respectively, $H(Y,Y')$ is the joint entropy of   $Y$ and $Y'$. This together with the invariance property of mutual information, i.e. $I(Z;Z') = I(Y;Y')$ under homeomorphisms condition, results in Theorem 1.

\section{Proof of Theorem 2}\label{app:B}%下面的对过了
Let $\tilde{Z}=\left[Z^{T}, Z^{\prime T}\right]^{T} \in \mathbb{R}^{2 d}$, and from (3), the joint distribution ${p_{Z,Z'}}(z,z')$ is $\tilde{Z} \sim \mathcal{G N}\left(\tilde{Z} ; \mu_{\tilde{Z}}, \Sigma_{\tilde{Z} \tilde{Z}}, \beta\right)$, where $\mu_{\tilde{Z}}$ is the mean, and $\Sigma_{\tilde{Z} \tilde{Z}}$ is the dispersion matrix. The MI between $Z$ and $Z^{\prime}$ is given by
\begin{align*}
& I\left(Z, Z^{\prime}\right)\\
&=\iint p_{Z, Z^{\prime}}\left(z, z^{\prime}\right) \log \frac{p_{Z, Z^{\prime}}\left(z, z^{\prime}\right)}{p_Z(z) p_{Z^{\prime}}\left(z^{\prime}\right)} d z d z^{\prime} \tag{12} \\ 
& =E\left[\log p_{Z, Z^{\prime}}\left(z, z^{\prime}\right)\right]-E\left[\log p_Z(z)\right]-E\left[\log p_{Z^{\prime}}\left(z^{\prime}\right)\right].
\end{align*}
Then, it follows that
$$
\begin{aligned}
& E\left[\log p_{Z, Z^{\prime}}\left(z, z^{\prime}\right)\right] \\
& =\log \frac{\Phi(\beta, 2 n)}{\left[\operatorname{det}\left(\Sigma_{\tilde{Z}\tilde{Z}}\right)\right]^{1 / 2}}-\frac{1}{2} E\left\{\left[\left(\tilde{Z}-\mu_{\tilde{Z}}\right)^{T} \Sigma_{\tilde{Z} \tilde{Z}}^{-1}\left(\tilde{Z}-\mu_{\tilde{Z}}\right)\right]^{\beta}\right\}
\end{aligned},
$$
where the expectation over the parameter space $\mathbb{R}^{n}$ of a function $\varphi\left((\tilde{Z}-\mu_{\tilde{Z}})^{T} \Sigma_{\tilde{Z}\tilde{Z}}^{-1}\left(\tilde{Z}-\mu_{\tilde{Z}}\right)\right)=\varphi\left(\Bar{Z}^{T} \Bar{Z}\right) \equiv \varphi(w)$ (with $w>0$ for $\left.\tilde{Z}-\mu_{\tilde{Z}} \neq 0\right)$ is essentially type 1 Dirichlet integral, which can be converted into integral over $\mathbb{R}^{+}$ \cite{verdoolaegeGeometryMultivariateGeneralized2012}. Specifically, let $\varphi(w)=w^{\beta}$, then

$$
\begin{aligned}
& E\left\{\left[\left(\tilde{Z}-\mu_{\tilde{Z}}\right)^{T} \Sigma_{\tilde{Z} \tilde{Z}}^{-1}\left(\tilde{Z}-\mu_{\tilde{Z}}\right)\right]^{\beta} \right\}\\
& =\frac{\Phi(\beta, 2 n)}{\left[\operatorname{det}\left(\Sigma_{\tilde{Z} \tilde{Z}}\right)\right]^{1 / 2}} \int_{\mathbb{R}^{2 n}}\left[\left(\tilde{Z}-\mu_{\tilde{Z}}\right)^{T} \Sigma_{\tilde{Z} \tilde{Z}}^{-1}\left(\tilde{Z}-\mu_{\tilde{Z}}\right)\right]^{\beta}\\ &~~~~~~~\times\exp \left(-\frac{1}{2}\left[\left(\tilde{Z}-\mu_{\tilde{Z}}\right)^{T} \Sigma_{\tilde{Z} \tilde{Z}}^{-1}\left(\tilde{Z}-\mu_{\tilde{Z}}\right)\right]^{\beta}\right) d \tilde{z} \\
& \stackrel{(a)}{=} \frac{\beta}{2^{n / \beta} \Gamma(n / \beta)} \int_{\mathbb{R}^{+}} \varphi(w) w^{n-1} \exp \left(-\frac{1}{2} w^{\beta}\right) d w \\
& =\frac{\beta}{2^{n / \beta} \Gamma(n / \beta)} \frac{2^{2+n / \beta} \Gamma\left((\beta+n) / \beta\right)}{2 \beta} \\
& =\frac{2 \Gamma((\beta+n) / \beta)}{\Gamma(n / \beta)}\\
&=\frac{2 n}{\beta}
\end{aligned},
$$

where (a) is due to the fact that the density function of the positive variable $w=\left(\tilde{Z}-\mu_{\tilde{Z}}\right)^{T} \Sigma_{\tilde{Z} \tilde{Z}}^{-1}\left(\tilde{Z}-\mu_{\tilde{Z}}\right)$ is given by \cite{verdoolaegeGeometryMultivariateGeneralized2012}

$$
p(w ; \beta)=\frac{\beta}{\Gamma\left(\frac{n}{\beta}\right) 2^{\frac{n}{\beta}}} w^{n-1} \exp \left(-\frac{1}{2} w^{\beta}\right).
$$

Therefore,

$$
E\left[\log p_{Z, Z^{\prime}}\left(z,z ^{\prime}\right)\right]=\log \frac{\Phi(\beta, 2 n)}{\left[\operatorname{det}\left(\Sigma_{\tilde{Z} \tilde{Z}}\right)\right]^{1 / 2}}-\frac{2 n}{\beta}.
$$

Similarly,

$$
\begin{gathered}
E\left[\log p_{Z}(z)\right]=\log \frac{\Phi(\beta, n)}{\left[\operatorname{det}\left(\Sigma_{ZZ}\right)\right]^{1 / 2}}-\frac{n}{\beta}, \\
E\left[\log p_{Z^{\prime}}\left(z^{\prime}\right)\right]=\log \frac{\Phi(\beta, n)}{\left[\operatorname{det}\left(\Sigma_{Z^{\prime} Z^{\prime}}\right)\right]^{1 / 2}}-\frac{n}{\beta}.
\end{gathered}
$$

Substituting these expectations into (7) leads to


\begin{align*}
& I\left(Z, Z^{\prime}\right) \\
& =\frac{1}{2} \log \frac{\operatorname{det}\left(\Sigma_{Z Z}\right) \operatorname{det}\left(\Sigma_{Z^{\prime} Z^{\prime}}\right)}{\operatorname{det}\left(\Sigma_{\tilde{Z} \tilde{Z}}\right)}+\log \frac{\Phi(\beta, 2 n)}{[\Phi(\beta, n)]^{2}}  \tag{13}\\
& =\frac{1}{2} \log \frac{\operatorname{det}\left(\Sigma_{Z Z}\right) \operatorname{det}\left(\Sigma_{Z^{\prime} Z^{\prime}}\right)}{\operatorname{det}\left(\Sigma_{\tilde{Z} \tilde{Z}}\right)},
\end{align*}


where we used $\Phi(\beta, n)=\frac{\beta \Gamma(n / 2)}{2^{n /(2 \beta)} \pi^{n / 2} \Gamma(n /(2 \beta))}$ and the following relation

$$
\frac{\Phi(\beta, 2 n)}{[\Phi(\beta, n)]^{2}}=\frac{\beta \Gamma(n)}{\Gamma(n / \beta)} \frac{\left[\Gamma\left(\frac{n}{2 \beta}\right)\right]^{2}}{\left[\beta \Gamma\left(\frac{n}{2}\right)\right]^{2}}=\frac{1}{\beta} \frac{2^{n-\frac{1}{2}}}{2^{\frac{n}{\beta}-\frac{1}{2}}} \frac{\Gamma\left(\frac{n}{2}+\frac{1}{2}\right)}{\Gamma\left(\frac{n}{2 \beta}+\frac{1}{2}\right)} \frac{\Gamma\left(\frac{n}{2 \beta}\right)}{\Gamma\left(\frac{n}{2}\right)}=1.
$$

Then, using the relation between the dispersion matrix and covariance matrix


\begin{equation*}
{\Sigma _{\tilde X\tilde X}}{\rm{ = }}\frac{{n\Gamma (n/(2\beta ))}}{{{2^{1/\beta }}\Gamma ((n + 2)/(2\beta ))}}{C_{\tilde X\tilde X}},
% \Sigma_{\ddot{x} \ddot{x}}=\frac{n \Gamma(n /(2 \beta))}{2^{1 / \beta} \Gamma((n+2) /(2 \beta))} C_{\ddot{x} \tilde{x}}, \tag{14}
\end{equation*}


it follows that

$$
I\left(Z ; Z^{\prime}\right)=\frac{1}{2} \log \frac{\operatorname{det}\left(\Sigma_{ZZ}\right) \operatorname{det}\left(\Sigma_{Z^{\prime} Z^{\prime}}\right)}{\operatorname{det}\left(\Sigma_{\tilde{Z} \tilde{Z}}\right)}=\frac{1}{2} \log \frac{\operatorname{det}\left(C_{Z Z}\right) \operatorname{det}\left(C_{Z^{\prime} Z^{\prime}}\right)}{\operatorname{det}\left(C_{\tilde{Z} \tilde{Z}}\right)}.
$$

\section{ Experiment Implementation Details} \label{app:C}
% For lack of computation resources, we run with 1020 batch size on 3 A100 GPUs for 100 and 400 epoch, and run with 1024 batch size on 4 V100 GPUS for 800 epochs. We run the pretrain process with 16-bit precision. And we employ 4 batches of gradient accumulation to stabilize model updating when the determination has relatively high dimensions as well as to speed up the training process. Note that this is not equivalent to increasing batch size. 
For experiments on ImageNet-1K, we use a batch size of 1020 on 3 A100 GPUs for 100, 400, and 800 epochs. %, and a batch size of 1024 across 4 V100 GPUs for 800 epochs. 
Training is conducted using 16-bit precision (FP16) and 4 batches of gradient accumulation to stabilize model updating and accelerate the training process. We use the LARS optimizer with a base learning rate of 0.8 for the backbone pretraining and 0.2 for the classifier training. The learning rate is scaled by $ \text{lr} = \text{base\_lr}  \times \text{batch\_size}  /  256 \times \text{num\_gpu} $.  We use a weight decay of 1.5E-6 for backbone parameters. 
The linear classifier is trained on top of frozen backbone. We follow the default setting as in Solo-learn benchmark \cite{costaSololearnLibrarySelfsupervised2022} for the rest of the training hyper-parameters.  

For our method with a momentum encoder, we follow the setting of \cite{grillBootstrapYourOwn2020,chenExploringSimpleSiamese2020} 
and use a two-layer predictor with hidden dimension 1024 for all datasets. %and update the average of eigenvalues of $C_{ZZ}$ every 1000 batches with a moving average coefficient $\rho$ of 0.1 to track the eigenvalues used for the rescaling operation (\ref{rescaling}). 
For ImageNet-100, we set the base learning rate as 0.2 for backbone pretraining and 0.3 for the classifier. We set the weight decay of backbone parameters as 0.0001. 
For CIFAR-100, we set the base learning rate for backbone pretraining as 0.3 and the classifier as 0.2. The weight decay is set as 6E-5. For the rescaling operation (\ref{rescaling}), we track the eigenvalues of $C_{ZZ}$ with an update interval of 100 batches with a moving average coefficient $\rho$ of 0.99.
% The average of eigenvalues of $C_{ZZ}$ is updated every 1000 epochs with a moving average coefficient $\rho$ of 0. The other hyperparameters are default settings in solo-learn benchmark\cite{costaSololearnLibrarySelfsupervised2022}. 
%For momentum encoder based training on ImageNet100, we set the base learning rate of 0.3 for backbone and classifier. The weight decay parameter remains 0.0001. For CIFAR-100 plain training, we set the base learning rate for backbone as 0.3 and the classifier as 0.2. The weight decay is set as 6e-5. The average of eigenvalues of $C_{ZZ}$ is updated every 100 epochs with a moving average coefficient $\rho$ of 0.99. For CIFAR-100 momentum training, we set the base learning rate for backbone as 0.3 and the classifier as 0.2. The weight decay is set as 1e-4. 
Table \ref{tab:update-ema-CIFAR-100-Table} shows the ablation study on the update interval and moving average coefficient $\rho$. Generally, a larger update interval should be used with a smaller moving average coefficient, and vice versa. This is reasonable as the two parameters together control the speed of the eigenvalue tracking.
Overall, our method is insensitive to these two hyperparameters.

Table \ref{tab:beta-cifar100} and Figure \ref{fig:abl_beta} depict the ablation study on the parameter $\beta$ used for the rescaling operation (\ref{rescaling}). We adhere to the experimental setup described in Table \ref{tab:CIFAR_linear} and report the Top-1 accuracy on CIFAR-100. As shown in Table \ref{tab:beta-cifar100} and Figure \ref{fig:abl_beta}, a smaller $\beta$ results in faster convergence during training. However, excessively small values may lead to training failure. We set $\beta=5$ for all the experiments. 
\begin{table}[h]
    \caption{Ablation study on the update interval and moving average coefficient $\rho$ for eigenvalues tracking used for the rescaling operation (\ref{rescaling}).}
        \vspace{\baselineskip} % 在标题前添加近似单行间距
    \label{tab:update-ema-CIFAR-100-Table}
    \centering
    \begin{tabular}{lcc}
      \toprule
      update interval & $\rho$ & CIFAR-100 \\
      \midrule
      1000 & 0 & 69.45 \\
      1000 & 0.1 & 70.22 \\
      1000 & 0.99 & 68.69 \\
      100 & 0.99 & 70.54 \\
      1 & 0.99 & 69.17 \\
      1 & 0 & 69.37 \\
      \bottomrule
    \end{tabular}
  \end{table}
  
\begin{table}[h]
  \caption{{Ablation study on the parameter $\beta$ used for the rescaling operation (\ref{rescaling})}. }
      \vspace{\baselineskip} % 在标题前添加近似单行间距
  \label{tab:beta-cifar100}
  \centering
  \begin{tabular}{cc}
    \toprule
   ${\beta}$ & {CIFAR-100} \\
    \midrule
    % 10 & 69.39 \\
    7  & 69.85 \\
    6  & 70.10 \\
    5  & 70.17 \\
    4  & 70.09 \\
    3  & 69.46 \\
    1  &$ \mathrm{NaN} $\\
    \bottomrule
  \end{tabular}
\end{table}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.8\linewidth]{contents//figs//exps/beta_acc1.png}
    \caption{The convergence curves of our method on CIFAR-100 for different values of the parameter $\beta$ used for the rescaling operation (\ref{rescaling}).}
    \label{fig:abl_beta}
\end{figure}

\subsection*{C. ImageNet Pre-train}
512batch size, ema0, update interval 1000,dim4096, lr 2.4, cls lr: 0.4, wd 1.5e-6,  pred: 1024, 70.33
71.28, lr0.8 
\subsection{Gradient Accumulation}



